RecipeQA: A Challenge Dataset for Multimodal Comprehension of Cooking Recipes

Understanding and reasoning about cooking recipes is a fruitful research direction towards enabling machines to interpret procedural text. In this work, we introduce RecipeQA, a dataset for multimodal comprehension of cooking recipes. It comprises of approximately 20K instructional recipes with multiple modalities such as titles, descriptions and aligned set of images. With over 36K automatically generated question-answer pairs, we design a set of comprehension and reasoning tasks that require joint understanding of images and text, capturing the temporal flow of events and making sense of procedural knowledge. Our preliminary results indicate that RecipeQA will serve as a challenging test bed and an ideal benchmark for evaluating machine comprehension systems. The data and leaderboard are available at http://hucvl.github.io/recipeqa.

==> etc/05.analysis.tex <==
\subsection{Dataset Statistics}
In the previous month we looked at the dataset statistics and how the recipes are formed. These statistics enabled us to understand our dataset in an exploratory manner. For instance we could know understand our dataset better, such as how many recipes we have at hand, how many steps do these recipes contain, and the average number of steps in a recipe as well as the image and title distribution \emph{etc}.

We also wanted to better understand the word level statistics for two modalities we have at hand. In particular, we wanted to see the distribution of words in the recipe descriptions as well as the recipe titles. In order to do that we generated word clouds for both of these modalities. In the following we provide those statistics.

\subsection{Traing Validation Test Splits}

\vspace{-2mm}
\begin{table}[ht]
\label{tab:cbt_stat}
  \begin{center}
    {\small 
      {\sc 
        \begin{tabular}{lccc}
          & Training & Validation & Test \\
          \hline
          %\hline
          Number of books & 98 & 5 & 5 \\
          Number of questions (context+query)& 669,343 & 8,000 & 10,000  \\
          Average words in contexts & 465 & 435 & 445 \\
          Average words in queries & 31 & 27 & 29 \\
          Distinct candidates & 37,242 & 5,485 & 7,108 \\
          \hline
          %Vocabulary size & \multicolumn{3}{c}{53,628}\\
          %\hline
        \end{tabular}
      }
    }
    \caption{\label{tab:cbt_stat} {\bf Statistics of the CBT.} Breakdown by question class is provided with the data set files.}
  \end{center}
\vspace*{-4ex}
\end{table}

\textbf{This is just a placeholder taken from the CBT paper.
}

\subsubsection{Word Clouds}

%\includegraphics[width=\textwidth]{word_title.png}
Here put two figures.

%\includegraphics[width=\textwidth]{word_desc.png}

\subsubsection{Word Distribution}

Here provide other examples.

\subsubsection{Look at the report for more details}

Here provide other examples. Especially from other datasets.

==> etc/tbl3.tex <==
\begin{table*}[!htb]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lllllll}
\hline
Dataset        & Image Source & \multicolumn{1}{c}{Question Source} & Formulation & \#Images     & \#Questions & Modality         \\ \hline
%SQuAD          & -            & Human                               & RC          & -            & 100K        & Text             \\
%MCTest         & -            & Human                               & RC          & -            & 2640        & Text             \\
%WikiQA         & -            & Query Logs                          & IR          & -            & 3047        & Text             \\
%TREC-QA        & -            & Query Logs                          & IR          & -            & 1479        & Text             \\
%CNN/Daily Mail & -            & Summary + Cloze                     & RC          & -            & 1.4M        & Text             \\
%CBT            & -            & Cloze                               & RC          & -            & 688K        & Text             \\
%DAQUAR         & NYU-Depth V2 & Human                               & VQA         & 1,449        & 12,468      & Image            \\
%Visual Madlibs & COCO         & Human                               & VQA         & 10,738       & 360,001     & Image            \\
%VQA            & COCO         & Human                               & VQA         & 204,721      & 614,163     & Image            \\
%COCO-QA        & COCO         & Syntetic                            & VQA         & 117,684      & 117,684     & Image            \\
%FM-IQA         & COCO         & Human                               & VQA         & 158,392      & 14,944      & Image            \\
%Visual7W       & COCO         & Human                               & VQA         & 47,300       & 327,939     & Image            \\
%CLEVR          & Rendered     & Syntetic                            & VQA         & 100,000      & 999,968     & Image            \\
%FigureQA       & Plotted      & Syntetic                            & VQA         & 100,000 (Figures) & 1M     & Image/Text       \\
COMICS         & Comics       & Cloze, Coherence                    & COMICS      & 1.2M  & 750K       & Image/Text       \\
MovieQA        & Movies       & Human                               & Movie QA    & 408  & 14,944      & Image/Video/Text \\
TQA            & CK12         & Human                               & TQA         & 3,455        & 26,260      & Image/Text       \\

%       &              &                                     &             &              &             &                  \\ %\hline
RecipeQA       & Recipes     & Cloze, Coherence, Ordering        & RecipeQA    & 95015      & 36784             & Image/Text            \\
%               &              &                                     &             &              &             &                  \\ 
\hline
\end{tabular}
}
\caption{A Summary of Multimodal Machine Comprehension Datasets}
\label{tbl:datasetcomparison}
\end{table*}
